GeoNLF: Geometry guided Pose-Free Neural LiDAR Fields

Although recent efforts have extended Neural Radiance Fields (NeRF) into LiDAR point cloud synthesis, the majority of existing works exhibit a strong dependence on precomputed poses. However, point cloud registration methods struggle to achieve precise global pose estimation, whereas previous pose-free NeRFs overlook geometric consistency in global reconstruction. In light of this, we explore the geometric insights of point clouds, which provide explicit registration priors for reconstruction. Based on this, we propose Geometry guided Neural LiDAR Fields(GeoNLF), a hybrid framework performing alternately global neural reconstruction and pure geometric pose optimization. Furthermore, NeRFs tend to overfit individual frames and easily get stuck in local minima under sparse-view inputs. To tackle this issue, we develop a selective-reweighting strategy and introduce geometric constraints for robust optimization. Extensive experiments on NuScenes and KITTI-360 datasets demonstrate the superiority of GeoNLF in both novel view synthesis and multi-view registration of low-frequency large-scale point clouds.

==> More_Content_and_Deprecated/3_1_preliminaries_.tex <==
\subsection{Preliminaries}
\label{sec:preliminaries}
\textbf{NeRF and pose-free NeRF}. NeRF represents a 3D scene implicitly though a mapping function $F_\Theta=F_\Theta^{'} \circ \gamma$ and the entire process of synthesizing novel views can be summarized as "map-then-integrate". For a ray cast from a pixel of the novel view image, NeRF samples a sequence of points $\mathbf{p_i} \in \mathbb{R}^{5}: (\mathbf{x_i},\theta,\phi)$, where the $\mathbf{x_i} \in \mathbb{R}^{3}$ and $(\theta,\phi)$ is the viewing direction. Then NeRFs map the 5D input into higher dimensional space though positional encoding.The $L_{th}$ layer is denoted as $\gamma^{trg}_L$ in vanilla NeRF and $\gamma^{hash}_L$ in iNGP~\cite{muller2022instant}:

\begin{align}
    %\gamma_{trg}(p) = (\sin(2^0\pi p), (\cos(2^0\pi p), (\sin(2^{L-1}\pi p),(\cos(2^{L-1}\pi p),
    \gamma^{trg}_L(x) = ((\sin(2^{L-1}\pi x),(\cos(2^{L-1}\pi x)), \qquad \gamma^{hash}_L(x) = \mathrm{TriLinear}(\mathcal{H}_L,x)
    \label{eq:volume_rendering}
\end{align}

where $\mathcal{H}_l \in \mathbb{R}^{d\times d\times d \times f}$ is the hash grid with $d$ spatial resolution and $f$ feature channels. The final position encoding is the concatenation of features from $L$ layers.Then the map-then-integrate process can be described as follows: first, applying a mapping function $F_\Theta^{'} \to (\mathbf{c},\sigma)$ to obtain a radiance color $c \in \mathbb{R}^3$ and a volume density value $\sigma$, then integrating along the ray to derive the RGB value of the pixel:

\begin{align}
    \hat{\mathcal C}(\mathbf{r}) = \sum_{i=1}^NT_i(1-e^{-\sigma_i\delta_i}) \mathbf c_i, \qquad  T_i = \exp ( -\sum_{j=1}^{i-1}\sigma_j\delta_j )
    \label{eq:volume_rendering}
\end{align}

where $T$ indicates the accumulated transmittance, $\delta$ refers to the distance between samples. Finally, given $M$ images $\mathcal{I}=\{I_i | i=0,1...,N-1\}$ with camera poses $P=\{P_s | s=0,1...N-1\}$, we can optimize NeRFs by minimizing the error $\mathcal{L} = \sum_i^N \|\hat{I}_i-I_i\|^2_2$ between the rendered image $\hat{I}$ and the ground truth image $I$More Content/Deprecated:

\begin{align}
    \Theta^*=\arg \min _{\Theta} \mathcal{L}(\hat{\mathcal{I}} \mid \mathcal{I}, P)
    \label{eq:volume_rendering}
\end{align}

While NeRF requires precise camera parameters as input, pose-free NeRF only uses images $\mathcal{I}=\{I_i | i=0,1...,N-1\}$ as input, simply treating the camera parameters $P=\{P_s | s=0,1...N-1\}$ as learnable parameters similar to $\Theta$. Hence, the simultaneous update of P and theta via gradient descent transforms the optimization objective of NeRF to:

\begin{align}
    \Theta^*, \mathcal{P}^*=\arg \min _{\Theta,\mathcal{P}} \mathcal{L}(\hat{\mathcal{I}},\hat{\mathcal{P}} \mid \mathcal{I})
    \label{eq:volume_rendering}
\end{align}

\textbf{Coarse-to-fine registration for bundle adjusting NeRF}. Inspired by the coarse-to-fine registration, BARF~\cite{lin2021barf} and a series of subsequent works~\cite{heo2023robust,chen2023dbarf,truong2023sparf,liu2023robust}  demonstrate the applicability of the coarse-to-fine strategy to pose-free NeRF. A mask is applied to reweight the $L_{th}$ positional encoding:
\begin{align}
    \gamma_L'(\mathbf{x} ; \alpha)=w_L(\alpha)\gamma_L
    \label{eq:volume_rendering}
\end{align}

where the weight $w_L(\alpha)$ is defined as:

\begin{align}
    w_L(\alpha)= \begin{cases}0 & \text { if } \alpha<L \\ \frac{1-\cos ((\alpha-L) \pi)}{2} & \text { if } 0 \leq \alpha-L<1 \\ 1 & \text { if } \alpha-L \geq 1\end{cases}
\end{align}

$\alpha \in \left[ 0, L \right]$ is a controllable parameter proportional to the optimization progress. Consequently, the weight gradually becomes 1 from the coarsest resolution(iNGP) or lowest frequency(vanilla NeRF) to the finest resolution or highest frequency. This strategy has also been adopted in our pipeline.

% \textbf{Problem Formulation}.
% %尽管Bundle adjusting
% In the large-scale outdoor driving scenario, given the collected LiDAR point cloud sequence $\mathcal{S}=\{S_i | i=0,1...,N-1\}$ with



